Transfer Learning Study of Motion Transformer-based Trajectory Predictions

Trajectory planning in autonomous driving is highly dependent on predicting the emergent behavior of other road users. Learning-based methods are currently showing impressive results in simulation-based challenges, with transformer-based architectures technologically leading the way. Ultimately, however, predictions are needed in the real world. In addition to the shifts from simulation to the real world, many vehicle- and country-specific shifts, i.e. differences in sensor systems, fusion and perception algorithms as well as traffic rules and laws, are on the agenda. Since models that can cover all system setups and design domains at once are not yet foreseeable, model adaptation plays a central role. Therefore, a simulation-based study on transfer learning techniques is conducted on basis of a transformer-based model. Furthermore, the study aims to provide insights into possible trade-offs between computational time and performance to support effective transfers into the real world.

==> img/plots_amcm/result-plots.tex <==
Formatting still needs some work, but here are the results.

% Some confusing abbreviations are used here to keep the horizontal width of this table in
% check. See the xtick and xticklabels parameters in any of the following plots for a map
% from these abbreviations to their spelled-out counterparts.
\pgfplotstableread[row sep=\\,col sep=&]{
    ivl & S mAP  & S minADE & S minFDE & S MissRate & T mAP  & T minADE & T minFDE & T MissRate \\
    blt & 0.0917 &   4.6698 &  10.2989 &     0.6901 & 0.2078 &   2.4123 &   5.2653 &     0.4720 \\
    bls & 0.3968 &   0.8880 &   1.6266 &     0.1723 & 0.2947 &   1.5261 &   3.4756 &     0.3152 \\
    mtl & 0.3290 &   0.8864 &   1.6550 &     0.1647 & 0.2391 &   1.9461 &   4.2792 &     0.3923 \\
    tlw & 0.1774 &   1.9257 &   3.4042 &     0.3973 & 0.6611 &   0.6508 &   1.2165 &     0.0782 \\
    tld & 0.1887 &   1.6017 &   3.0359 &     0.3794 & 0.4413 &   0.9639 &   1.7298 &     0.1802 \\
    tle & 0.1925 &   1.8823 &   3.4256 &     0.3914 & 0.4968 &   0.8308 &   1.6501 &     0.1669 \\
    tlf & 0.1928 &   1.4524 &   2.7074 &     0.3588 & 0.3785 &   1.2275 &   2.4087 &     0.2684 \\
    }\results

\begin{figure*}[htbp!]
\centering
\begin{tikzpicture}
    \begin{axis}[
            ybar,
            symbolic x coords={blt, bls, mtl, tlw, tld, tle, tlf},
            xtick=data,
            xtick={blt, bls, mtl, tlw, tld, tle, tlf},
            xticklabels={
            	Baseline (target only),
            	Baseline (source only),
            	Multi-task Learning,
            	Transfer Learning: whole model fine-tuning,
            	Transfer Learning: decoder fine-tuning,
            	Transfer Learning: encoder fine-tuning,
            	Transfer Learning: feature-based
            },
            xticklabel style={rotate=45, anchor=east},
            width=0.6\textwidth,
            height=0.4\textwidth,
            ymin=0,
            ylabel={mAP},
            legend pos=outer north east,
            legend cell align={left},
            grid=both,
            grid style={dotted,gray!80}
        ]
        \addplot table[x=ivl,y=T mAP]{\results};
        \addplot table[x=ivl,y=S mAP]{\results};
        \legend{Target mAP, Source mAP}
    \end{axis}
\end{tikzpicture}
\caption{Comparison of training approaches based on mAP.}
\label{fig:results_mAP}
\end{figure*}

\begin{figure*}[htbp!]
\centering
\begin{tikzpicture}
    \begin{axis}[
            ybar,
            symbolic x coords={blt, bls, mtl, tlw, tld, tle, tlf},
            xtick=data,
            xtick={blt, bls, mtl, tlw, tld, tle, tlf},
            xticklabels={
            	Baseline (target only),
            	Baseline (source only),
            	Multi-task Learning,
            	Transfer Learning: whole model fine-tuning,
            	Transfer Learning: decoder fine-tuning,
            	Transfer Learning: encoder fine-tuning,
            	Transfer Learning: feature-based
            },
            xticklabel style={rotate=45, anchor=east},
            width=0.6\textwidth,
            height=0.4\textwidth,
            ymin=0,
            ylabel={minADE},
            legend pos=outer north east,
            legend cell align={left},
            grid=both,
            grid style={dotted,gray!80}
        ]
        \addplot table[x=ivl,y=T minADE]{\results};
        \addplot table[x=ivl,y=S minADE]{\results};
        \legend{Target minADE, Source minADE}
    \end{axis}
\end{tikzpicture}
\caption{Comparison of training approaches based on minADE.}
\label{fig:results_minADE}
\end{figure*}

\begin{figure*}[htbp!]
\centering
\begin{tikzpicture}
    \begin{axis}[
            ybar,
            symbolic x coords={blt, bls, mtl, tlw, tld, tle, tlf},
            xtick=data,
            xtick={blt, bls, mtl, tlw, tld, tle, tlf},
            xticklabels={
            	Baseline (target only),
            	Baseline (source only),
            	Multi-task Learning,
            	Transfer Learning: whole model fine-tuning,
            	Transfer Learning: decoder fine-tuning,
            	Transfer Learning: encoder fine-tuning,
            	Transfer Learning: feature-based
            },
            xticklabel style={rotate=45, anchor=east},
            width=0.6\textwidth,
            height=0.4\textwidth,
            ymin=0,
            ylabel={minFDE},
            legend pos=outer north east,
            legend cell align={left},
            grid=both,
            grid style={dotted,gray!80}
        ]
        \addplot table[x=ivl,y=T minFDE]{\results};
        \addplot table[x=ivl,y=S minFDE]{\results};
        \legend{Target minFDE, Source minFDE}
    \end{axis}
\end{tikzpicture}
\caption{Comparison of training approaches based on minFDE.}
\label{fig:results_minFDE}
\end{figure*}

\begin{figure*}[htbp!]
\centering
\begin{tikzpicture}
    \begin{axis}[
            ybar,
            symbolic x coords={blt, bls, mtl, tlw, tld, tle, tlf},
            xtick=data,
            xtick={blt, bls, mtl, tlw, tld, tle, tlf},
            xticklabels={
            	Baseline (target only),
            	Baseline (source only),
            	Multi-task Learning,
            	Transfer Learning: whole model fine-tuning,
            	Transfer Learning: decoder fine-tuning,
            	Transfer Learning: encoder fine-tuning,
            	Transfer Learning: feature-based
            },
            xticklabel style={rotate=45, anchor=east},
            width=0.6\textwidth,
            height=0.4\textwidth,
            ymin=0,
            ylabel={MissRate},
            legend pos=outer north east,
            legend cell align={left},
            grid=both,
            grid style={dotted,gray!80}
        ]
        \addplot table[x=ivl,y=T minADE]{\results};
        \addplot table[x=ivl,y=S minADE]{\results};
        \legend{Target MissRate, Source MissRate}
    \end{axis}
\end{tikzpicture}
\caption{Comparison of training approaches based on MissRate.}
\label{fig:results_MissRate}
\end{figure*}

==> src/99_Evaluation_old.tex <==
\section{EVALUATION}\label{analysis}

%\begin{itemize}
% By this point, reader has seen source/target domain, transformer
%    \item description of datasets
%    \item overall software architecture
%    \item results table, quantitative visualizations?
%    \item hardware setup, computation time
%appendix: visual example(s)
%\end{itemize}

%Here should be practical realization insights, information about setup, how we conducted it.

%Evaluation is more that just the metrics, we should also include computation time, parameters etc. to make %it more solid, such that we really provide some benefiting contribution to the community.

%Here could be also a place to considere initial validation test, that have been done, nevertheless, %results, plots tables could be switched to appendix (create new section if appendiy is needed)

%It's worth rethinking the visualization. Could we visualize it more differently/ diverse? Would table %structure save space?

This section provides experimental results and relevant context. First, the the source and target datasets are described. Second, an overview of the software architecture used for data synthesis, model training and evaluation is given. Evaluation results are provided next, followed finally by a description of the hardware and the required processing time.

\subsection{Datasets}

% NOTE: I like using text and figure here because it is thorough (via the text) and it conveys the size difference (via the figure). I tried using a table when writing the thesis paper but didn't find it as clear.

% \pgfplotstableread[row sep=\\,col sep=&]{
%     ivl  & Training & Validation & Testing \\
%     WOMD & 2144874  & 192172     & 196050  \\  
%     CMD  & 134480   & 27785      & 28668   \\  
%     }\datasets

% \begin{figure}[ht!]
% \centering
% \begin{tikzpicture}
%     \begin{axis}[
%             ybar stacked,
%             xtick=data,
%             ylabel=\# of trajectories,
%             bar width=0.1\textwidth,
%             enlarge x limits=1,
%                 legend style={
%                         cells={anchor=west},
%                         legend pos=north east,
%                 },
%                 reverse legend=true,
%                 xticklabels from table={\datasets}{ivl},
%                 %xticklabel style={text width=2cm, align=center},
%         ]
%         \addplot table [y=Testing, meta=ivl, x expr=\coordindex]{\datasets};
%         \addlegendentry{Testing}
%         \addplot table [y=Validation, meta=ivl, x expr=\coordindex]{\datasets};
%         \addlegendentry{Validation}
%         \addplot table [y=Training, meta=ivl, x expr=\coordindex]{\datasets     };  
%         \addlegendentry{Training}
%     \end{axis}
% \end{tikzpicture}
% \caption{Relative sizes of the source and target datasets, with training/validation/testing splits.}
% \label{fig:datasets}
% \end{figure}

% \subsubsection{Waymo Open Motion Dataset}

% The Waymo Open Motion Dataset (WOMD) is used as the source dataset for domain adaptation. The WOMD consists of 575,205 sample scenarios each containing 9 seconds of data. These samples encompass 2,566,096 distinct trajectories. Of these samples, 487,005 are designated for training, 44,100 for validation and 44,100 for testing, representing a split of 84\% for training, 8\% for validation and 8\% for testing. This dataset captures trajectories of vehicles, cyclists, and pedestrians in proportions of roughly 70\%, 7\%, and 23\%, respectively. Each trajectory is a sequence of states sampled at 10Hz. Every state describes the agent's center point in 3D coordinates, bounding box dimensions, velocity vector (X and Y coordinates), and direction.

% \subsubsection{CarMaker Dataset}

% The CMD is used as the target dataset for domain adaptation. It comprises 190,933 trajectories of 9 seconds each, with a training/validation/test split of 70\%, 15\% and 15\%, respectively. Trajectories are represented in the same manner as in the WOMD. That is, each trajectory consists of a sequence of states, with each state reporting the agent's center point in 3D coordinates, bounding box dimensions, velocity vector (X and Y coordinates), and direction. Unlike the WOMD, the CMD only contains vehicle trajectories. This is because CarMaker has limited behavior synthesis capabilities for pedestrians and cyclists, making it impractical to generate realistic trajectories for these agent types at sufficient scale.



\subsection{Results}



Quantitative evaluation results are provided in Table \ref{tab:results}, using prediction scoring metrics defined by Waymo \cite{ettinger2021large}. The highest performance on the target dataset is acheived by the fine-tuned model, by a significant margin across all metrics. This is demonstrated visually in Figure \ref{fig:T3}, which shows the fine-tuned model more closely predicting a vehicle's trajectory when preparing to turn through an intersection in the target dataset. However, the fine-tuned model performs worse on the source dataset than the source-only baseline from which it is derived, indicating the presence of catastrophic forgetting \cite{kirkpatrick2017overcoming}. A visual example of this is shown in Figure \ref{fig:S2}, which shows the source-only baseline model more closely predicting a vehicle's trajectory when preparing to turn through an intersection in the source dataset.

% \begin{figure}[ht]
% \begin{subfigure}{.4\textwidth}
%         \centering
%         \includegraphics[width=0.4\linewidth]{img/scenarios/T3S.png}
%         \caption{Source-only baseline model.}
%         \label{fig:T3S}
% \end{subfigure}
% \begin{subfigure}{.4\textwidth}
%         \centering
%         \includegraphics[width=0.4\linewidth]{img/scenarios/T3F.png}
%         \caption{Fine-tuned model.}
%         \label{fig:T3F}
% \end{subfigure}
% \caption{Target dataset (CMD): vehicle waiting at the edge of an intersection, preparing to make a right turn. The focus vehicle and its ground truth trajectory are green, while its predicted trajectories are red. Neighboring vehicles and their ground truth trajectories are blue, while their predicted trajectories are purple.}
% \label{fig:T3}
% \end{figure}

\begin{figure}
	\centering	
	\begin{subfigure}{0.46\textwidth}
		\includegraphics[width=\linewidth]{img/scenarios/T3S.png}
		\caption{Source-only baseline model.}
        \label{fig:T3S}
	\end{subfigure}
	\begin{subfigure}{0.46\textwidth}
		\includegraphics[width=\linewidth]{img/scenarios/T3F.png}
		\caption{Fine-tuned model.}
        \label{fig:T3F}
	\end{subfigure}
	\caption{Target dataset (CMD): vehicle waiting at the edge of an intersection, preparing to make a right turn. The focus vehicle and its ground truth trajectory are green, while its predicted trajectories are red. Neighboring vehicles and their ground truth trajectories are blue, while their predicted trajectories are purple.}
\end{figure}

\begin{figure}[]
\begin{subfigure}
        \centering
        \includegraphics[scale=0.26]{img/scenarios/T3S.png}
        \caption{Source-only baseline model.}
        \label{fig:T3S}
\end{subfigure}
\begin{subfigure}
        \centering
        \includegraphics[]{img/scenarios/T3F.png}
        \caption{Fine-tuned model.}
        \label{fig:T3F}
\end{subfigure}
\caption{Target dataset (CMD): vehicle waiting at the edge of an intersection, preparing to make a right turn. The focus vehicle and its ground truth trajectory are green, while its predicted trajectories are red. Neighboring vehicles and their ground truth trajectories are blue, while their predicted trajectories are purple.}
\label{fig:T3}
\end{figure}

% \begin{figure}[ht]
% \begin{subfigure}{.4\textwidth}
%         \centering
%         \includegraphics[width=0.6\linewidth]{img/scenarios/S2S.png}
%         \caption{Source-only baseline model.}
%         \label{fig:S2S}
% \end{subfigure}
% \begin{subfigure}{.4\textwidth}
%         \centering
%         \includegraphics[width=0.6\linewidth]{img/scenarios/S2F.png}
%         \caption{Fine-tuned model.}
%         \label{fig:S2F}
% \end{subfigure}
% \caption{Source dataset (WOMD): vehicle waits for another vehicle to pass before making a right turn. The focus vehicle and its ground truth trajectory are green, while its predicted trajectories are red. Neighboring vehicles and their ground truth trajectories are blue, while their predicted trajectories are purple.}
% \label{fig:S2}
% \end{figure}

Catastrophic forgetting is mitigated by fine-tuning only the encoder or the decoder, at the cost of lower performance on the target dataset. Fine-tuning the encoder results in generally better performance than fine-tuning the decoder, with better results on all target dataset metrics as well as mAP on the source dataset. This is an unexpected result, since the encoder contains only 8\% of the MTR model's total trainable parameters, with the other 92\% comprising the decoder. This offers a clue that the encoder may be more likely to capture domain-specific features, while the decoder operates on more general features.

% TODO: note in conclusion that this is a possible subject for further research

One notable feature of the results in Table \ref{tab:results} is that performance is generally higher on the target dataset than on the source dataset. This is expected, since the target dataset is less complex than the source dataset: not only does the target dataset contain fewer samples, it also represents a less detailed domain, since any simulated environment can be assumed to be less detailed than the reality it simulates.

% TODO: note in conclusion that further research could try using more data?

\pgfplotstableread[row sep=\\,col sep=&]{
    ivl & S mAP  & S minADE & S minFDE & S MissRate & T mAP  & T minADE & T minFDE & T MissRate \\
    blt & 0.0917 &   4.6698 &  10.2989 &     0.6901 & 0.2078 &   2.4123 &   5.2653 &     0.4720 \\
    bls & 0.3968 &   0.8880 &   1.6266 &     0.1723 & 0.2947 &   1.5261 &   3.4756 &     0.3152 \\
    mtl & 0.3290 &   0.8864 &   1.6550 &     0.1647 & 0.2391 &   1.9461 &   4.2792 &     0.3923 \\
    tlw & 0.1774 &   1.9257 &   3.4042 &     0.3973 & 0.6611 &   0.6508 &   1.2165 &     0.0782 \\
    tld & 0.1887 &   1.6017 &   3.0359 &     0.3794 & 0.4413 &   0.9639 &   1.7298 &     0.1802 \\
    tle & 0.1925 &   1.8823 &   3.4256 &     0.3914 & 0.4968 &   0.8308 &   1.6501 &     0.1669 \\
    tlf & 0.1928 &   1.4524 &   2.7074 &     0.3588 & 0.3785 &   1.2275 &   2.4087 &     0.2684 \\
    }\results

\newcommand{\computemax}[2]{
    \pgfplotstablesort[sort key={#1},sort cmp={float >}]{\sorted}{\results}
    \pgfplotstablegetelem{0}{#1}\of{\sorted}
    \pgfmathsetmacro{#2}{\pgfplotsretval}
}
\computemax{S mAP}{\maxSmAP}
\computemax{T mAP}{\maxTmAP}

\newcommand{\computemin}[2]{
    \pgfplotstablesort[sort key={#1},sort cmp={float <}]{\sorted}{\results}
    \pgfplotstablegetelem{0}{#1}\of{\sorted}
    \pgfmathsetmacro{#2}{\pgfplotsretval}
}
\computemin{S minADE}{\minSminADE}
\computemin{S minFDE}{\minSminFDE}
\computemin{S MissRate}{\minSMissRate}
\computemin{T minADE}{\minTminADE}
\computemin{T minFDE}{\minTminFDE}
\computemin{T MissRate}{\minTMissRate}


\begin{table*}[ht]
\centering
\caption{Evaluation of domain adaptation techniques.}
\begin{adjustbox}{max width=\textwidth}
\pgfplotstabletypeset[
    columns={ivl, S mAP, S minADE, S minFDE, S MissRate, T mAP, T minADE, T minFDE, T MissRate},
    columns/ivl/.style={string replace={ivl={}}, column name={},string type},
    columns/S mAP/.style={fixed, precision=4, column name=mAP, postproc cell content/.append code={\ifdim##1 pt=\maxSmAP pt\relax \pgfkeysalso{@cell content=\bfseries##1} \fi}},
    columns/S minADE/.style={fixed, precision=4, column name=minADE, postproc cell content/.append code={\ifdim##1 pt=\minSminADE pt\relax \pgfkeysalso{@cell content=\bfseries##1} \fi}},
    columns/S minFDE/.style={fixed, precision=4, column name=minFDE, postproc cell content/.append code={\ifdim##1 pt=\minSminFDE pt\relax \pgfkeysalso{@cell content=\bfseries##1} \fi}},
    columns/S MissRate/.style={fixed, precision=4, column name=MissRate, postproc cell content/.append code={\ifdim##1 pt=\minSMissRate pt\relax \pgfkeysalso{@cell content=\bfseries##1} \fi}},
    columns/T mAP/.style={fixed, precision=4, column name=mAP, postproc cell content/.append code={\ifdim##1 pt=\maxTmAP pt\relax \pgfkeysalso{@cell content=\bfseries##1} \fi}},
    columns/T minADE/.style={fixed, precision=4, column name=minADE, postproc cell content/.append code={\ifdim##1 pt=\minTminADE pt\relax \pgfkeysalso{@cell content=\bfseries##1} \fi}},
    columns/T minFDE/.style={fixed, precision=4, column name=minFDE, postproc cell content/.append code={\ifdim##1 pt=\minTminFDE pt\relax \pgfkeysalso{@cell content=\bfseries##1} \fi}},
    columns/T MissRate/.style={fixed, precision=4, column name=MissRate, postproc cell content/.append code={\ifdim##1 pt=\minTMissRate pt\relax \pgfkeysalso{@cell content=\bfseries##1} \fi}},
    every head row/.style={
        before row={%
            \toprule
            & \multicolumn{4}{c}{Source Dataset} & \multicolumn{4}{c}{Target Dataset} \\
            \cmidrule(lr){2-5} \cmidrule(lr){6-9}
        },
        after row={\midrule}
    },
    every last row/.style={after row=\bottomrule},
    every row 0 column 0/.style={postproc cell content/.style={@cell content={Baseline: Target-only }}},
    every row 1 column 0/.style={postproc cell content/.style={@cell content={Baseline: Source-only}}},
    every row 2 column 0/.style={postproc cell content/.style={@cell content={MTL}}},
    every row 3 column 0/.style={postproc cell content/.style={@cell content={Fine-tuned}}},
    every row 4 column 0/.style={postproc cell content/.style={@cell content={Fine-tuned Decoder}}},
    every row 5 column 0/.style={postproc cell content/.style={@cell content={Fine-tuned Encoder}}},
    every row 6 column 0/.style={postproc cell content/.style={@cell content={Feature Reuse}}},
]{\results}
\end{adjustbox}
\label{tab:results}
\end{table*}

\subsection{Hardware and Training Duration}

Performance is irrelevant if the technique is so resource intensive as to be infeasible. Therefore, all training in this paper is performed using a desktop computer with a single GPU. Specifically, a workstation PC with a single NVIDIA A5000 GPU. In the source-only baseline, target-only baseline, and MTL experiments, the model is trained on its entire training dataset all at once. In the fine-tuned, fine-tuned decoder, fine-tuned encoder, and feature reuse experiments the model is trained first on the source dataset (this is equivalent to the source-only baseline) and is then trained on the target dataset. This is an important distinction, because whereas experiments in the first category always require the full training time, experiments in the second category only require training on the source dataset once, after which each experiment may start from this common intermediate stage. Figure \ref{fig:training_time} shows the total training time required for each model. Figure \ref{fig:tuning_time} shows the time required for training on the target dataset only, for applicable models.

\pgfplotstableread[row sep=\\,col sep=&]{
    ivl & Duration \\
    %Source-only baseline & 16.02    \\
    %Target-only baseline & 0.961    \\
    %Multi-task learning  & 19.17    \\
    %Fine-tuned           & 16.98    \\
    %Fine-tuned decoder   & 16.94    \\
    %Fine-tuned encoder   & 16.75    \\
    %Feature Reuse        & 16.35    \\
    SOB & 16.02    \\
    TOB & 0.961    \\
    MTL & 19.17    \\
    FT  & 16.98    \\
    FTD & 16.94    \\
    FTE & 16.75    \\
    FR  & 16.35    \\
    }\trainingtime

\begin{figure}[ht!]
\centering
\begin{tikzpicture}
    \begin{axis}[
            ybar,
            xtick=data,
            width=0.45\textwidth,
            height=0.26\textwidth,
            %symbolic x coords={Source-only baseline, Target-only baseline, Multi-task learning, Fine-tuned, Fine-tuned decoder, Fine-tuned encoder, Feature Reuse},
            symbolic x coords={SOB, TOB, MTL, FT, FTD, FTE, FR},
            xticklabel style={rotate=45, anchor=east},
            ylabel={Training time in days}
            %bar width=0.1\textwidth,
            %enlarge x limits=1,
                %xticklabels from table={\trainingtime}{ivl},
                %xticklabel style={text width=2cm, align=center},
        ]
        \addplot table [y=Duration]{\trainingtime};
    \end{axis}
\end{tikzpicture}
\caption{Total training duration for each model.}
\label{fig:training_time}
\end{figure}

\pgfplotstableread[row sep=\\,col sep=&]{
    ivl & Duration \\
    %Fine-tuned           & 0.96    \\
    %Fine-tuned decoder   & 0.92    \\
    %Fine-tuned encoder   & 0.73    \\
    %Feature Reuse        & 0.33    \\
    FT  & 0.96    \\
    FTD & 0.92    \\
    FTE & 0.73    \\
    FR  & 0.33    \\
    }\tuningtime

\begin{figure}[ht!]
\centering
\begin{tikzpicture}
    \begin{axis}[
            ybar,
            xtick=data,
            width=0.45\textwidth,
            height=0.26\textwidth,
            %symbolic x coords={Fine-tuned, Fine-tuned decoder, Fine-tuned encoder, Feature Reuse},
            symbolic x coords={FT, FTD, FTE, FR},
            xticklabel style={rotate=45, anchor=east},
            ylabel={Training time in days}
            %bar width=0.1\textwidth,
            %enlarge x limits=1,
                %xticklabels from table={\trainingtime}{ivl},
                %xticklabel style={text width=2cm, align=center},
        ]
        \addplot table [y=Duration]{\tuningtime};
    \end{axis}
\end{tikzpicture}
\caption{Transfer learning training duration for each model.}
\label{fig:tuning_time}
\end{figure}

==> src/99_IEEE_info.tex <==
\section{IEEE Info}

\subsection{Maintaining the Integrity of the Specifications}

The IEEEtran class file is used to format your paper and style the text. All margins, 
column widths, line spaces, and text fonts are prescribed; please do not 
alter them. You may note peculiarities. For example, the head margin
measures proportionately more than is customary. This measurement 
and others are deliberate, using specifications that anticipate your paper 
as one part of the entire proceedings, and not as an independent document. 
Please do not revise any of the current designations.

\section{Prepare Your Paper Before Styling}
Before you begin to format your paper, first write and save the content as a 
separate text file. Complete all content and organizational editing before 
formatting. Please note sections \ref{AA}--\ref{SCM} below for more information on 
proofreading, spelling and grammar.

Keep your text and graphic files separate until after the text has been 
formatted and styled. Do not number text heads---{\LaTeX} will do that 
for you.

\subsection{Abbreviations and Acronyms}\label{AA}
Define abbreviations and acronyms the first time they are used in the text, 
even after they have been defined in the abstract. Abbreviations such as 
IEEE, SI, MKS, CGS, ac, dc, and rms do not have to be defined. Do not use 
abbreviations in the title or heads unless they are unavoidable.

\subsection{Units}
\begin{itemize}
\item Use either SI (MKS) or CGS as primary units. (SI units are encouraged.) English units may be used as secondary units (in parentheses). An exception would be the use of English units as identifiers in trade, such as ``3.5-inch disk drive''.
\item Avoid combining SI and CGS units, such as current in amperes and magnetic field in oersteds. This often leads to confusion because equations do not balance dimensionally. If you must use mixed units, clearly state the units for each quantity that you use in an equation.
\item Do not mix complete spellings and abbreviations of units: ``Wb/m\textsuperscript{2}'' or ``webers per square meter'', not ``webers/m\textsuperscript{2}''. Spell out units when they appear in text: ``. . . a few henries'', not ``. . . a few H''.
\item Use a zero before decimal points: ``0.25'', not ``.25''. Use ``cm\textsuperscript{3}'', not ``cc''.)
\end{itemize}

\subsection{Equations}
Number equations consecutively. To make your 
equations more compact, you may use the solidus (~/~), the exp function, or 
appropriate exponents. Italicize Roman symbols for quantities and variables, 
but not Greek symbols. Use a long dash rather than a hyphen for a minus 
sign. Punctuate equations with commas or periods when they are part of a 
sentence, as in:
\begin{equation}
a+b=\gamma\label{eq}
\end{equation}

Be sure that the 
symbols in your equation have been defined before or immediately following 
the equation. Use ``\eqref{eq}'', not ``Eq.~\eqref{eq}'' or ``equation \eqref{eq}'', except at 
the beginning of a sentence: ``Equation \eqref{eq} is . . .''

\subsection{\LaTeX-Specific Advice}

Please use ``soft'' (e.g., \verb|\eqref{Eq}|) cross references instead
of ``hard'' references (e.g., \verb|(1)|). That will make it possible
to combine sections, add equations, or change the order of figures or
citations without having to go through the file line by line.

Please don't use the \verb|{eqnarray}| equation environment. Use
\verb|{align}| or \verb|{IEEEeqnarray}| instead. The \verb|{eqnarray}|
environment leaves unsightly spaces around relation symbols.

Please note that the \verb|{subequations}| environment in {\LaTeX}
will increment the main equation counter even when there are no
equation numbers displayed. If you forget that, you might write an
article in which the equation numbers skip from (17) to (20), causing
the copy editors to wonder if you've discovered a new method of
counting.

{\BibTeX} does not work by magic. It doesn't get the bibliographic
data from thin air but from .bib files. If you use {\BibTeX} to produce a
bibliography you must send the .bib files. 

{\LaTeX} can't read your mind. If you assign the same label to a
subsubsection and a table, you might find that Table I has been cross
referenced as Table IV-B3. 

{\LaTeX} does not have precognitive abilities. If you put a
\verb|\label| command before the command that updates the counter it's
supposed to be using, the label will pick up the last counter to be
cross referenced instead. In particular, a \verb|\label| command
should not go before the caption of a figure or a table.

Do not use \verb|\nonumber| inside the \verb|{array}| environment. It
will not stop equation numbers inside \verb|{array}| (there won't be
any anyway) and it might stop a wanted equation number in the
surrounding equation.

\subsection{Some Common Mistakes}\label{SCM}
\begin{itemize}
\item The word ``data'' is plural, not singular.
\item The subscript for the permeability of vacuum $\mu_{0}$, and other common scientific constants, is zero with subscript formatting, not a lowercase letter ``o''.
\item In American English, commas, semicolons, periods, question and exclamation marks are located within quotation marks only when a complete thought or name is cited, such as a title or full quotation. When quotation marks are used, instead of a bold or italic typeface, to highlight a word or phrase, punctuation should appear outside of the quotation marks. A parenthetical phrase or statement at the end of a sentence is punctuated outside of the closing parenthesis (like this). (A parenthetical sentence is punctuated within the parentheses.)
\item A graph within a graph is an ``inset'', not an ``insert''. The word alternatively is preferred to the word ``alternately'' (unless you really mean something that alternates).
\item Do not use the word ``essentially'' to mean ``approximately'' or ``effectively''.
\item In your paper title, if the words ``that uses'' can accurately replace the word ``using'', capitalize the ``u''; if not, keep using lower-cased.
\item Be aware of the different meanings of the homophones ``affect'' and ``effect'', ``complement'' and ``compliment'', ``discreet'' and ``discrete'', ``principal'' and ``principle''.
\item Do not confuse ``imply'' and ``infer''.
\item The prefix ``non'' is not a word; it should be joined to the word it modifies, usually without a hyphen.
\item There is no period after the ``et'' in the Latin abbreviation ``et al.''.
\item The abbreviation ``i.e.'' means ``that is'', and the abbreviation ``e.g.'' means ``for example''.
\end{itemize}
An excellent style manual for science writers is \cite{b7}.



\subsection{Identify the Headings}
Headings, or heads, are organizational devices that guide the reader through 
your paper. There are two types: component heads and text heads.

Component heads identify the different components of your paper and are not 
topically subordinate to each other. Examples include Acknowledgments and 
References and, for these, the correct style to use is ``Heading 5''. Use 
``figure caption'' for your Figure captions, and ``table head'' for your 
table title. Run-in heads, such as ``Abstract'', will require you to apply a 
style (in this case, italic) in addition to the style provided by the drop 
down menu to differentiate the head from the text.

Text heads organize the topics on a relational, hierarchical basis. For 
example, the paper title is the primary text head because all subsequent 
material relates and elaborates on this one topic. If there are two or more 
sub-topics, the next level head (uppercase Roman numerals) should be used 
and, conversely, if there are not at least two sub-topics, then no subheads 
should be introduced.

\subsection{Figures and Tables}
\paragraph{Positioning Figures and Tables} Place figures and tables at the top and 
bottom of columns. Avoid placing them in the middle of columns. Large 
figures and tables may span across both columns. Figure captions should be 
below the figures; table heads should appear above the tables. Insert 
figures and tables after they are cited in the text. Use the abbreviation 
``Fig.~\ref{fig}'', even at the beginning of a sentence.

\begin{table}[htbp]
\caption{Table Type Styles}
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Table}&\multicolumn{3}{|c|}{\textbf{Table Column Head}} \\
\cline{2-4} 
\textbf{Head} & \textbf{\textit{Table column subhead}}& \textbf{\textit{Subhead}}& \textbf{\textit{Subhead}} \\
\hline
copy& More table copy$^{\mathrm{a}}$& &  \\
\hline
\multicolumn{4}{l}{$^{\mathrm{a}}$Sample of a Table footnote.}
\end{tabular}
\label{tab1}
\end{center}
\end{table}

\begin{figure}[htbp]
\centerline{\includegraphics{fig1.png}}
\caption{Example of a figure caption.}
\label{fig}
\end{figure}

Figure Labels: Use 8 point Times New Roman for Figure labels. Use words 
rather than symbols or abbreviations when writing Figure axis labels to 
avoid confusing the reader. As an example, write the quantity 
``Magnetization'', or ``Magnetization, M'', not just ``M''. If including 
units in the label, present them within parentheses. Do not label axes only 
with units. In the example, write ``Magnetization (A/m)'' or ``Magnetization 
\{A[m(1)]\}'', not just ``A/m''. Do not label axes with a ratio of 
quantities and units. For example, write ``Temperature (K)'', not 
``Temperature/K''.


\section*{References}

Please number citations consecutively within brackets \cite{b1}. The 
sentence punctuation follows the bracket \cite{b2}. Refer simply to the reference 
number, as in \cite{b3}---do not use ``Ref. \cite{b3}'' or ``reference \cite{b3}'' except at 
the beginning of a sentence: ``Reference \cite{b3} was the first $\ldots$''

Number footnotes separately in superscripts. Place the actual footnote at 
the bottom of the column in which it was cited. Do not put footnotes in the 
abstract or reference list. Use letters for table footnotes.

Unless there are six authors or more give all authors' names; do not use 
``et al.''. Papers that have not been published, even if they have been 
submitted for publication, should be cited as ``unpublished'' \cite{b4}. Papers 
that have been accepted for publication should be cited as ``in press'' \cite{b5}. 
Capitalize only the first word in a paper title, except for proper nouns and 
element symbols.

For papers published in translation journals, please give the English 
citation first, followed by the original foreign-language citation \cite{b6}.

\begin{thebibliography}{00}
\bibitem{b1} G. Eason, B. Noble, and I. N. Sneddon, ``On certain integrals of Lipschitz-Hankel type involving products of Bessel functions,'' Phil. Trans. Roy. Soc. London, vol. A247, pp. 529--551, April 1955.
\bibitem{b2} J. Clerk Maxwell, A Treatise on Electricity and Magnetism, 3rd ed., vol. 2. Oxford: Clarendon, 1892, pp.68--73.
\bibitem{b3} I. S. Jacobs and C. P. Bean, ``Fine particles, thin films and exchange anisotropy,'' in Magnetism, vol. III, G. T. Rado and H. Suhl, Eds. New York: Academic, 1963, pp. 271--350.
\bibitem{b4} K. Elissa, ``Title of paper if known,'' unpublished.
\bibitem{b5} R. Nicole, ``Title of paper with only first word capitalized,'' J. Name Stand. Abbrev., in press.
\bibitem{b6} Y. Yorozu, M. Hirano, K. Oka, and Y. Tagawa, ``Electron spectroscopy studies on magneto-optical media and plastic substrate interface,'' IEEE Transl. J. Magn. Japan, vol. 2, pp. 740--741, August 1987 [Digests 9th Annual Conf. Magnetics Japan, p. 301, 1982].
\bibitem{b7} M. Young, The Technical Writer's Handbook. Mill Valley, CA: University Science, 1989.
\end{thebibliography}
\vspace{12pt}
\color{red}
IEEE conference templates contain guidance text for composing and formatting conference papers. Please ensure that all template text is removed from your conference paper prior to submission to the conference. Failure to remove the template text from your paper may result in your paper not being published.

==> src/99_MTR_old.tex <==
\section{MOTION TRANSFORMER }\label{motion_transformer}



The Motion Transformer (MTR) is a model architecture that has achieved state of the art results in trajectory prediction for autonomous driving, scoring 1st on the Waymo Motion Prediction Challenge 2022 \cite{bib:shi2022mtra}. 


The original transformer was developed for the problem of machine translation \cite{bib:vaswani2023attention}. It is divided into two components: an encoder, which maps inputs into a latent representation, and a decoder, which derives outputs from this latent representation. MTR, while based on the original transformer architecture, contains a variety of enhancements tailored to the problem of trajectory prediction. Unlike machine translation, in which a model operates in the space of a particular alphabet, trajectory prediction is a spatial problem. Furthermore, trajectory prediction is an inherently temporal problem, since the same trajectory over two different timescales implies different dynamics, whereas machine translation is not concerned with time at all. Another key difference is multimodality. There may be many possible ways to translate a sentence, but in general it is not important for a model to be able to produce more than one at a time. On the other hand, a vehicle approaching an intersection may proceed through the intersection in many possible ways (e.g. straight, left turn, right turn). Although that vehicle must eventually proceed in only one of these ways, more than one may be possible at prediction time, which means they all must be accounted for in trajectory prediction.

One particular challenge that MTR is designed to address is that of endpoint selection. There are two traditional approaches to endpoint selection. The more straightforward of the two, called direct regression, involves predicting trajectories directly without any prior assumption as to the location of the endpoint. While this method is straightforward to implement and unconstrained by the presence of spatial priors, it tends to result in slow convergence \cite{varadarajan2021multipath} \cite{ngiam2022scene}. The other approach, a class of methods referred to as “goal-based”, uses a spatial grid to reduce the number of endpoints considered. Trajectories are then regressed for each goal candidate within this spatial grid. Goal-based methods generally converge faster than direct regression, but the chosen density of the spatial grid presents a trade-off between convergence speed and performance, since a sparse grid corresponds to a low-fidelity sampling of the endpoint space, which limits the precision of the endpoint selection process \cite{bib:gu2021densetnt2, bib:zhao2020tnt}.

MTR introduces a new approach, called the “motion query pair”, which blends the goal-based concept with direct regression. The central idea of this approach is to have two queries rather than the traditional one. These are referred to as the static intention query and the dynamic searching query.

The static intention query $Q_{I}$ corresponds to the goal-based approach. However, rather than being drawn from a grid, the endpoint is drawn from a set of representative intention points $I$ determined by applying k-means clustering on a collection of ground truth trajectories from a training dataset. The query $Q_{I}$ is calculated by applying sinusoidal position encoding \cite{bib:vaswani2023attention} followed by an multi-layer perceptron (MLP) to this set.

\begin{align}
\label{eq:si_query}
                Q_{I} = MLP(PE(I))
\end{align}

The dynamic searching query $Q_{S}$ corresponds to direct regression. It is calculated for each of the model's 6 decoder layers in turn, by applying sinusoidal position encoding followed by an MLP to the predicted endpoint $Y_{T}$ from the previous layer.

\begin{align}
\label{eq:ds_query}
                Q_{S}^{j} = MLP(PE(Y_{T}^{j-1}))
\end{align}

The two queries are then fused during the multi-head self-attention (MHA) step as shown in (\ref{eq:mqp1}-\ref{eq:mqp4}). First, a multi-head self-attention block is applied to the query content features from the $(j-1)$-th decoder layer $C^{j-1}$ and the static intention query, yielding an intermediate query content representation $C_{sa}^j$.

\begin{equation}
    \begin{split}
    \label{eq:mqp1}
            C_{sa}^{j} & = MHA(query=C^{j-1} + Q_I, \\
            & key=C^{j-1} + Q_I, value=C^{j-1})
    \end{split}
\end{equation}

Then, additional multi-head attention blocks are used to aggregate agent features $C_A^j$ and map features $C_M^j$ from their respective base features $A$ and $M$, where $[\cdot, \cdot]$ represents feature concatenation and $\alpha(\cdot)$ represents a "dynamic map collection" operation that uses self-attention to emphasize the most relevant map features.

\begin{equation}
    \begin{split}
    \label{eq:mqp2}
            C_A^j & = MHA(query=[C_{sa}^j, Q_S^j], \\
            & key=[A, PE_A], value=A)
    \end{split}
\end{equation}

\begin{equation}
    \begin{split}
    \label{eq:mqp3}
            C_M^j = & MHA(query=[C_{sa}^j, Q_S^j], \\
            & key=[\alpha(M), PE_{\alpha(M)}], value=\alpha(M))
    \end{split}
\end{equation}

Finally the agent and map features are combined to yield the updated query content features $C^j$ for the j-th layer (\ref{eq:mqp4}).

\begin{align}
\label{eq:mqp4}
        C^j = MLP([C_A^j, C_M^j])
\end{align}

Another innovation of MTR is its ability to incorporate projected future interactions with neighboring agents into its predictions. This is done by adding a simple, low-cost trajectory prediction module within the encoder, which takes the encoded past agent features $A_{past}$ and passes them through an MLP to predict future agent position and velocity $S$ for each future timestep $1:T$.

\begin{align}
\label{eq:dense_future_prediction}
                S_{1:T} = MLP(A_{past})
\end{align}

These predicted future agent features are then concatenated with the past agent features before being passed to the decoder. This allows the decoder to make trajectory predictions based on both the known past agent state as well as a coarse prediction of future agent state, which in turn allows the model to incorporate predicted future agent interactions into its trajectory predictions. \cite{bib:shi2022mtra} shows with an ablation study that incorporation of these coarse predictions results in increased predictive performance.

==> src/XX_Notes.tex <==
\section{NOTES}

Questions:
\begin{itemize}
    \item Should we make the Background about MTR? --> No that's just a model
    \item Background should be about trajectory prediction trend evaluation in short with conclusion learning based
    \item handover to transfer learning by mentioning and shortly explaining current MTR outperforming
    \item Focus on Background should be on transfer learning techniques
    \item should we include the prestudies? e.g. in the appendix, i mean the validation stuff, done quite in the beginning
\end{itemize}

General structure:
\begin{itemize}
    \item Intro: Trajectory Prediction and transfer learning, first page max
    \item Background: ................., 1 page max (second page)
    \item Methodology: Different Approaches in transfer learning, 2 pages max
    \item Evaluation: Setup, Results, 2 page max
    \item Conclusion: Conclusion, really short paragraph
    \item Bib: 
\end{itemize}

´

==> src/intro_backup.tex <==

transformer related domain adaptation techniques are pre-investigated in Section Xy. The most promising methods are described in X and their results are presented in Y. 

and transformer related domain adaption techniques are introduced in Section \ref{related_work}. The selected motion transformer MTR and 

physical models of different
complexity are introduced in Section II. The methodology of CNP and the application to yaw rate prediction are described in Section III. Finally, CNP are evaluated in different scenarios and the results are compared with the various physical models in Section IV.






approaches haben sich in siluations-basierten 


Simulation-based development on basis of extensive challenge datasets provides a foundation for subsequent transfer. 


on which functionality can be transferred using small, dedicated datasets. 


Thus, a more feasible approach would be training on a large dataset followed by domain adaptation on smaller datasets, transferring functionality and performance to the specific domain and vehicle configuration at hand. 

As pointed out by \cite{karle2022scenario} learning based approaches (in their terminology pattern and planning base) are impressing but lacking real-world requirements. 



haben sich als Forschungsgrundlage etabliert. 

Waymo Open Motion Dataset, Agroverse, NuPlan, Shifts.
Lyft

Oxfort RoboCar ?

Lyft level 5 Prediction \cite{houston2021one}
ApolloScape Trajectory 
Agroverse Forcasting \cite{chang2019argoverse}
nuScenes prediction task
NuPlan 
Waymo Motion Prediction
Waymo Interaction Prediction 
NTERACTION Dataset \cite{zhan2019interaction}
Shift \cite{malinin2021shifts}

similar metrics have emergt





worden, anhand welchen die Performance unterschiedlicher Ansätze vergleichen werden können. 




und repräsentiert neben der Wahrnehmung einen zentralen Forschungsbereich des autonomen Fahrens dar. 



Insbesondere learnbasierte Ansätze haben in den Vergangenen Jahren an großem Interesse und Aufsehen gesorgt. Traditionelle, vornehmlich physikalische 


pure statisticall models 



Autonomous vehicles operating in the real-world are 

core of decision making takes place in the context of trajectory planning. Operation in open-world requires operation in collabortively used space. Thus 




\begin{itemize}
    \item relevance of trajectory prediction for safe planning and trustworthy decision making
    \item demonstrating learning based approaches are outperforming
    \item highlighting transformers are leading technologically
    \item transfer from challenges to real application, requirements and challenges
    \item Multi-task learning, domain adaption, transfer learning, (domain generalization not forseenable)
    \item Requirements from application, real-time, resource limitations
\end{itemize}

Questions to answer
\begin{itemize}
    \item why motion transformer
    \item why model adaption, transfer-learning
    \item why this study
\end{itemize}

Aspects to consider
\begin{itemize}
    \item \textit{rule based approaches are limited, corner cases, real-world, open world, open long-tail distribution}
    \item physics based approaches would require model about others, even if model is available, decisions and control inputs are not obvious
    \item physics, velocity-vector based predictions are limited, neglecting context like maps, neglecting interactions
    \item \textit{learning based approaches are necessary/promissing}
    \item Trajectory Prediction mainly learning based
    \item inherent complexity of the task
    \item ...
    \item predictions have local uncertainty, probabilistic prediction
    \item predictions have global goal / behavioural decision uncertainty, multimodality
    \item behaviour is effected by evolving of the situation, namely the behaviour of others, interactive / joint prediction instead of marginal prediction
    \item behaviour of all depend on the situation/ context, context consideration, context encoding, context embedding, context tokens
    \item ...
    \item \textit{Research has been conducted on trajectory prediction on the basis of multiple datasets and challengens}
    \item ... 
    \item \textit{learning based approaches have limitations, e.g. closed-loop behaviour differently than open-loop in prediction; this is known and addressed by NuPlan challenge in closed loop consideration}
    \item \textit{(Latest results show, that performance in data set is significantly different than in closed loop and real world)?}
    \item \textit{data in real world are likely to be different; different countries, different rules and law enforcement areas, different sensor setups, differnt fusion algorithm versions}
    \item Some day we need to go into the real world, there are multiple shifts ahead. ODD, Vehicle, Sensor Setup etc.. Domain Adaption is crucial, Domain generalization not there yet, small datasets from dedicated ODD and setup forseenable, vehicle setup, ODD keeps same over lifetime (Assumption), Domain Adaption seams to be adequate solution for nearby future
    \item later one is currently underrepresented, since research focus more on task performance improvement, what is necessary and pleasent since data are available
    \item Question is how to do it? If we need to do it for multiple domains, costly, should evaluate performance maintaining and quick solution!
    \item Thus we should try to find out where the underlying generalization knowledge is in current motion transformeres! (slighly hint to encoder decodere only!) 
    \item shift challenge adress kind-off the task of shifts consideration! \textbf{Are there results that hint towards transfer learning?}
\end{itemize}

\begin{itemize}
    \item even large data can not be used: 1) different countries: different traffic rules, driving behavior, 2) different vehicle setup: vehicle dynamics, sensor setup, sensor fusion
    \item psychology reason we need to explore; at some point in time we need to go to the real world an must test.
    \item we have various different challenges, people ca quickly adopt but AI correctly not. But we have normally some data from application domain. And vehicle stay normally in this domain. Thus we could use a big data set from one country, one vehicle setup. And some data from the system and ODD at hand, for which we could tune the model. 
    \item building up the same dataset as Waymo ist too costly, too time intensive for each vehicle and ODD. General driving challenges are more ore less independent. People are able to transfer their knowlegde. We do it similary.
    \item thus, there will be a big need to transfer Models to various setups and ODD in the near feature.
    \item thus, investigating and accuratly (high precision) and fast teqchnique is crucial
    \item therefore we conduct a study on techniques to transfer learn. 
    \item as baseline the currently best approach MTR is used
\end{itemize}


Die trajektorienprädiktion anderer verkehrsteilnehmer ist für die Planung und Entscheidungsfindung im bereich des autonomen Fahrens von großer Bedeutung

- crucial for understanding situation and make safe decisions
- joint consideration observed agent states and road maps
- task is challenging, due to inherent  multimodal behaviours and complex scene environment

- two modes: 1) goal-based methods, 2) direct-regression methods
1) predict dense goal candidates to cover all possible destinations; then completing the full trajectory for all selected candidates; fewer candidates decrese performance; more candidates  increase computation and memory costs

2) predict directly trajectory set based on encodings covering agents future behaviour adaptively; flexibility in  predicting broad range of agent behaviours; generally converge slowly; as without spatial priors different motion modi could emerge from observed data; tend to predict most  frequent modes of training data, since frequent modes dominate optimization of the model

MTR-A: unifining framework; takes best of both aspects; novel: motion query pairs; model motion prediction as joint optimization fo following: i) global intention localization task, ii) local movement refinement. 

i) aims to roughly identify agent's intention for reaching higher efficiency 

ii) aims to adaptively refine each's intention's predicted trajectory for better accurancy.

Approach stabilizes training process without depending on dense goal candidates enables flexible and adaptive prediction by enabling local refinement for each motion mode

encode scene context features
polyline encoding

learned token features are customized for focal egent

query-centric seöf-attention

generally tokenization is crucial

temporal causality

multiple sets of intention queries

MTR, MTR+, MTR++

why learnable , why 8 seconds, than state-of the art



bekommt increasing attention in recent years due to and is important


safety? 

transfer also to different setups, 
while there could be minimum requirements stipulated, vehicle setup could be flexible, so different sensors in the perecption, differences in fusion are to be expacted as well. 

Motivieren, warum es eine individuelle study benötigt!
Motion transformer unterscheiden sich von anderen transformern. Das Anwendungsfeld ist so groß, dass Motion transformer keine super nische sind weshalb es gerechtfertigt ist eine individuelle Untersuchung zu machen.

research hints towards we need learning, pattern based approaches 

challenges of trajectory prediction
shift challenge adressing shifts!


Hier muss motiviert werden warum wir das brauchen und abgrenzen zu bestehenden studien!

Generally introduction is kind of four step section: 1) Motivation, 2) related Work 3) contribution 4) structure. 

Especially Motivation and related work goes hand in hand. Thereby conducting delimitation of the work. Contribution is clearly stated after motivating and refering to related work etc. pp. Structur closes this section!

literature review, in overal perspective of the paper. 

Refer test \cite{gopnik2004theory}. 


Contribution:
\begin{itemize}
    \item Evaluation of various Transler-learning tequnics
    \item Providing insights \& guidance in how setup relevant equivalence between source and target
    \item Speeding up development and transfer to real world
\end{itemize}
